Information-theoretic tools for parametrized coarse-graining of non-equilibrium extended systems

In this paper we focus on the development of new methods suitable for efficient and reliable coarse-graining of {\it non-equilibrium} molecular systems. In this context, we propose error estimation and controlled-fidelity model reduction methods based on Path-Space Information Theory, and combine it with statistical parametric estimation of rates for non-equilibrium stationary processes. The approach we propose extends the applicability of existing information-based methods for deriving parametrized coarse-grained models to Non-Equilibrium systems with Stationary States (NESS). In the context of coarse-graining it allows for constructing optimal parametrized Markovian coarse-grained dynamics, by minimizing information loss (due to coarse-graining) on the path space. Furthermore, the associated path-space Fisher Information Matrix can provide confidence intervals for the corresponding parameter estimators. We demonstrate the proposed coarse-graining method in a non-equilibrium system with diffusing interacting particles, driven by out-of-equilibrium boundary conditions.

==> ppmacros_basic.tex <==
%---------------------------------------------------------------------
%
% PP MACROS
%
\def\PPCOMM#1{{\sc Petr:}** \noindent{\sf {#1}} **}
\def\MAKCOMM#1{{\sc Markos:}** \noindent{\bf {#1}} **}
\def\rev{{\bf **REVISION} }
\def\endrev{{\bf **ENDREVISION} }


%\def\mathbb#1{{#1}}
%
% Special letters
%

\def\vareps{\varepsilon}

%
% Caligraphic letters
%
\def\Cc{\mathcal{C}}
\def\Dd{\mathcal{D}}
\def\Ee{\mathcal{E}}
\def\Ff{\mathcal{F}}
\def\Gg{\mathcal{G}}
\def\Hh{\mathcal{H}}
\def\Kk{\mathcal{K}}
\def\Ll{\mathcal{L}}
\def\Mm{\mathcal{M}}
\def\Nn{{\mathcal{N}}}
\def\Oo{\mathcal{O}}
\def\Pp{\mathcal{P}}
\def\Qq{\mathcal{Q}}
\def\Rr{{\mathcal{R}}}
\def\Ss{\mathcal{S}}
\def\Tt{\mathcal{T}}
\def\Vv{\mathcal{V}}
\def\Yy{\mathcal{Y}}
\def\Zz{\mathcal{Z}}

%
% Mathbb letters
%
\def\E{\mathbb{E}}
\def\J{\mathbb{J}}
\def\K{\mathbb{K}}
\def\N{\mathbb{N}}
\def\P{\mathbb{P}}
\def\R{\mathbb{R}}
\def\S{\mathbb{S}}
\def\T{\mathbb{T}}
\def\Z{\mathbb{Z}}

%
% Bold letters in Math style
%
\def\chibf{\mathbf{\chi}}
\def\et{\pmb{\eta}}

%
% Miscellaneous
%
%
% Integration vars
\def\d{d}
\def\dd{\,d}
\def\dx{\d x}
\def\dv{\d v}
\def\ddx{\dd x}
\def\ddv{\dd v}
\def\DT{\Delta t}

%
% Differential operators
\def\VEC#1{{\mathbf{#1}}}        % print in bf - use for vectors 
\def\EXP#1{e^{#1}}
\def\DET{\det}
\def\DIFF{{D}}
\def\GRAD{\nabla}
\def\LAP{\Delta}
\def\DIV{{\mathrm{div}}}
\def\CURL{{\mathrm{curl}}}
\def\curl{{\mathrm{curl}}}
\def\PD#1#2{\frac{\partial{#1}}{\partial{#2}}}
\def\DF#1#2{\frac{{\mathrm d}{#1}}{{\mathrm d}{#2}}}
\def\DDF#1#2{\frac{{\mathrm d}^2{#1}}{{\mathrm d}{#2}^2}}
\def\DIFF{\partial}
\def\FDIFF{\partial}
\def\PDER#1#2{{\mathrm{D}_{#1}{#2}}}
\def\DFUN#1{{{#1}'}}

%
% Probability 
%
\def\EXPEC#1{{\mathbb{E}\left[{#1}\right]}}
\def\EXPECT{{\mathbb{E}}}
\def\EXPECWRT#1#2{{\mathbb{E}_{#1}\left[{#2}\right]}}
\def\PROB#1{{\mathbb{P}\left({#1}\right)}}
\def\PROBSP{\mathcal{P}_1(\OMSPH)}
\def\PROBSPA{\mathcal{P}(\OMSPH)}
\def\RELENT#1#2{\Rr\left(#1|#2\right)}
\def\AVG#1{{<\!\!#1\!\!>}}
\def\VAR{\mathrm{Var}}
\def\COV{\mathrm{Cov}\,}
\def\MEAN{\mathbb{E}}

%
% Convergence and function spaces
%
\def\OM{\Omega}                  % Omega
\def\SPWP#1{W^{{#1}}}            % space W^{#1}
\def\SPWOP#1{W^{1,{#1}}}         % space W^{1,p}
\def\SPLP#1{L^{#1}}              % space L^p
\def\SPLT{L^2}                   % space L^2
\def\LSP{L^2(\Omega,\R^d)}
\def\LINF{L^{\infty}}
\def\HSP{H^1(\R^3)}
\def\BL{BL(\OMSPH)}
\def\OMSPH{\Omega\times\Sph^2}
\def\CHARFUN#1{\chi_{{#1}}}
\def\BALLX{{B(x)}}
\def\LNORM#1#2{\Vert\,#1\,\Vert_{#2}}
\def\WNORM#1#2{\vert\,#1\,\vert_{#2}}
\def\WEAKLYSTAR{\stackrel{\ast}{\rightharpoonup}}
\def\WEAKLY{{\rightharpoonup}}
\def\SCPROD#1#2{\langle {#1},{#2}\rangle}

%
% Punctuation in math mode
%
\def\SPACE{\;\;\;}          % use for spaces in formulae
\def\SSPACE{\;\;\;\;\;\;}   % use for even more spaces in formulae
\def\COMMA{\,,}             % use for commas at the ends of formulae
\def\PERIOD{\,.}            % use for periods at the ends of formulae
\def\SEP{{\,|\,}}           % use for seperator in set defs, like {x\in R \SEP

%
% References and numbers in tables
%
\def\VIZ#1{(\ref{#1})}      % use for references to formulae
\def\NUM#1{{\tt{#1}}}       % use for numbers that are comp. generated
\def\num#1{{\tt{#1}}}   


%
% Special symbols
%
\def\Im{i}
\def\REAL{\mathrm{Re}\,}
\def\IMAG{\mathrm{Im}\,}
\def\ARG{\mathrm{arg}\,}
\def\BIGO{\mathcal{O}}
\def\SMALLO{\mathrm{o}}
\def\CONST{\mathrm{const}}
\def\qed{$\Box$}
\def\QED{$\Box$}
\def\PROOF{\noindent{\sc Proof:}\ }
\def\sgn{\mathrm{sgn}\,}
\def\SGN{\mathrm{sgn}\,}

\def\AONE{\mathrm{(A1)}}
\def\ATWO{\mathrm{(A2)}}
\def\CPU{\mathrm{CPU}}

\def\PROD{\prod}
\def\HALF{\frac{1}{2}}
\def\Sph{{\S}}

\def\DET{\mathrm{det}\,}
\def\TR{\mathrm{Tr}\,}
\def\DIAG{\mathrm{diag}\,}
\def\DIAM{\mathrm{diam}\,}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}{Lemma}[section]
%\newtheorem{proposition}{Proposition}[section]
%\newtheorem{conjecture}{Conjecture}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{definition}{Definition}[section]




==> ppmacros_specific.tex <==
%
% Paper specific macros
%
%


\def\LAWEXACT{P}
\def\LAWAPPROX{Q}
\def\CONFNEW{\sigma'}

\def\st{\{\sigma_t\}_{t\ge 0}}
\def\ast{\{\widetilde\sigma_t\}_{t\ge 0}}
\def\PROCS{\st} 
\def\PROCSAPP{\ast} 
\def\PATHS{\LAWEXACT_{[0,T]}}
\def\PATHSAPP{\LAWAPPROX_{[0,T]}}
\def\PATHSAPPPAR{{{\LAWAPPROX}^\theta_{[0,T]}}}
\def\EQUIL{\mu_{\sigma}}
\def\EQUILAPP{\mu_{\widehat\sigma}}
\def\LOPER{\mathcal{L}}
\def\HOPER{\widehat{H}}

\def\FISHER{\mathbf{F}}

\def\RELENTR{\mathcal{R}}
\def\RELENT#1#2{\mathcal{R}\left({#1}\SEP{#2}\right)}
\def\ENTRATE#1#2{\mathcal{H}({#1}\SEP{#2})}


\def\CMIN{c_\mathrm{min}}

\def\COPP{\mathbf{P}}





% Coarse-graining papers
%
% Hamiltonians, CG potentials etc
\def\HAMS{H^{(s)}}
\def\HAML{H^{(l)}}
\def\BARHAMS{\bar{H}^{(s)}}
\def\BARHAML{\bar{H}^{(l)}}
\def\WHAML{\widetilde{H}^{(l)}}
\def\VS{V^{(s)}}
\def\VL{V^{(l)}}
\def\US{U^{(s)}}
\def\UL{U^{(l)}}
\def\HU{\widetilde{U}}
\def\BARUL{\bar{U}^{(l)}}

\def\BARIT#1{{\bar {#1}}}
\def\BARH{\BARIT{H}}
\def\BARHZ{\BARIT{H}^{(0)}}
\def\BARM{\BARIT{\mu}}
\def\BARMZ{\BARIT{\mu}^{(0)}}

%
% Lattices, configuration spaces, CG params
\def\QCELL{q_c}                     % alias for q in old notation
%\def\LATT{{\Lambda}}                % Lattice
\def\LATTN{{\Lambda}_N}             % Lattice with the size N subscripted
%\def\LATTC{{\bar{\Lambda}_{M}}}     % CG lattice
\def\LATT{{\Lambda}_N}
\def\LATTC{{\Lambda^{c}_{M}}}

\def\SPINSP{\Sigma}
\def\SPINSPC{\Sigma^c}
%\def\SIGMA{{\mathcal{S}}}           % Configuration space (all \sigma's)
\def\SIGMA{{\mathcal{S}_N}}
\def\STATESP{\Sigma}                % statespace (values of sigma(x))
\def\SIGMAC{\bar{\mathcal{S}}_{M}}  % CG config space
\def\NUMSP{{K}}                       % number of species

\def\COP{\mathbf{T}}                % CG operator
\def\COPI{\mathbf{R}}


%
% KMC related
%
\def\rej{\mathrm{rej}}
\def\NULL{\mathrm{null}}
\def\multi{\mathrm{multi}}
\def\SUCC{\mathrm{succ}}

%
% Probability & stochastic processes
%
\def\LOPER{\mathcal{L}}                                % Generator of a process 
\def\Es{\mathbb{E}_{\sigma_0}}                         % expectation conditions on initial state

\def\RELENTR#1#2{\mathcal{H}\left({#1}\SEP{#2}\right)}
\def\FISHER{\mathbf{F}_{\mathcal{R}}}
\def\FISHERR{\mathbf{F_{\mathcal{H}}}}
%\def\LAWEXACT{Q_{[0,T]}^{\theta}}
%\def\LAWAPPROX{Q_{[0,T]}^{\theta+\epsilon}}
%\def\PATHS{\LAWEXACT}
%\def\PATHSAPP{\LAWAPPROX}
\def\EQUIL{\mu^\theta}
\def\EQUILAPP{\mu^{\theta+\epsilon}}

%\def\LAWEXACT{Q_{[0,T]}^{\theta}}
%\def\LAWAPPROX{Q_{[0,T]}^{\theta+\epsilon}}
%\def\PATHS{\LAWEXACT}
%\def\PATHSAPP{\LAWAPPROX}
\def\EQUIL{\mu^\theta}
\def\EQUILAPP{\mu^{\theta+\epsilon}}


\def\st{\{\sigma_t\}_{t\ge 0}}
\def\ast{\{\widetilde\sigma_t\}_{t\ge 0}}
\def\PROCS{\st} 
\def\PROCSAPP{\ast} 
\def\PROCMICRO{\sigma_t}
\def\HS{\widetilde{\sigma}}
\def\HSt{\{\widetilde{\sigma_t}\}_{t\in[0,T]}}
\def\St{\{\sigma_t\}_{t\in[0,T]}}

\def\st{\{\sigma_t\}_{t\ge 0}}
\def\ast{\{\widetilde\sigma_t\}_{t\ge 0}}
\def\etat{\{\eta_t\}_{t\ge 0}}

\def\StT{\{\sigma_t\}_{t \in [0,T]}}
\def\ST{\{S_t\}_{t \in [0,T]}}
\def\aSttT{\{\tilde S_t\}_{t \in [0,T]}}
\def\aStT{\{\tilde \sigma_t\}_{t \in [0,T]}}
\def\muN{\mu_{N,\beta}}
\def\mutN{\widetilde\mu_{N,\beta}}

\def\HC{\widetilde{c}}
\def\HL{\widetilde{\lambda}}
\def\HLl{\widetilde{\Ll}}
\def\HQm{\widetilde {\Dd}_{[0,T]}}
\def\Qm{ {\Dd}_{[0,T]}}
\def\crf{c_{\mathrm{rf}}}
\def\trf{\mathrm{rf}}

\def\Csp{\{\sigma': \COP\sigma'=\eta'\}}
\def\Cspace{\{\sigma\in \Sigma\!: \COP\sigma=\eta\}}

\def\CMspace{\BARIT\Sigma_M}



